StablePrompt: Automatic Prompt Tuning using Reinforcement Learning for Large Language Models

Finding appropriate prompts for the specific task has become an important issue as the usage of Large Language Models (LLM) has expanded. Reinforcement Learning (RL) is widely used for prompt tuning, but its inherent instability and environmental dependency make it difficult to use in practice. In this paper, we propose StablePrompt, which strikes a balance between training stability and search space, mitigating the instability of RL and producing high-performance prompts. We formulate prompt tuning as an online RL problem between the agent and target LLM and introduce Adaptive Proximal Policy Optimization (APPO). APPO introduces an LLM anchor model to adaptively adjust the rate of policy updates. This allows for flexible prompt search while preserving the linguistic ability of the pre-trained LLM. StablePrompt outperforms previous methods on various tasks including text classification, question answering, and text generation. Our code can be found in github.

==> latex/intro_rollback.tex <==
First, we introduce Proximal Policy Optimization (PPO)~\cite{schulman2017proximal} as an RL optimizer. 
To build an Actor-Critic framework, we introduce a value head in Agent LLM and train it using PPO. 
We also use LoRA to effectively reduce the training parameters. 
This can be used on models larger than 7B, unlike RLprompt~\cite{deng2022rlprompt}, which trains a heavy MLP layer.

Second, we modify the KL-divergence term of the PPO objective for prompt tuning.
We introduce an anchor model and modify the objective term to ensure that the agent model does not diverge too much from the anchor model.
Anchor model is defined as the snapshot of the agent model at specific time.
We periodically compare the performance of the agent model to the anchor model and only update the anchor model if there is a significant improvement in performance.
By maintaining an anchor model with guaranteed performance improvements, it helps agent models to find better prompts more reliably.
 This approach, termed Adaptive PPO (APPO), strikes a balance between original PPO~\cite{schulman2017proximal} and RLHF-style PPO~\cite{ouyang2022training}, allowing reliable training without excessively restricting the search space.

Finally, we use the anchor model to implement an agent rollback method. If the agent model significantly underperforms compared to the anchor model, we rollback to the anchor model and retrain. This prevents incorrect training due to unstable indirect reward signals.

==> latex/tables/Agent_Target_Pair_Table.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{2}{*}{} & \multicolumn{4}{c}{Prompting Method} & \multicolumn{4}{c}{StablePrompt} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
        & No prompt & Manual Prompt & Few-shot Prompt & Few-shot Manual Prompt & gemma-2b & gemma-7b & mistral-7b & llama-3-8b \\
        \midrule
gemma-2b   & 55.3          & 51.0         & 54.3 &          61.6 &              62.5 &         63.1 &         62.5 &           61.7           \\
gemma-7b   & 61.7          & 71.2           & 65.3          & 72.8              & 73.6         & 76.0         & 75.4           & 74.9           \\
mistral-7b & 72.4          & 62.5           & 75.2          & 74.3              & 77.5         & 78.9         & 79.3           & 79.8           \\
llama-3-8b & 47.7          & 55.4           & 54.1          & 58.1              & 54.9         & 59.5         & 62.7           & 64.9           \\
falcon-11b & 63.2          & 70.9           & 72.1          & 73.8              & 74.8         & 78.8         & 78.7           & 78.2           \\ \bottomrule
\end{tabular}%
}
\caption{}
\label{}
\end{table*}
